BV-structures on the homology of the framed long knot space

We introduce BV-algebra structures on the homology of the space of framed long knots in $\mathbb{R}^n$ in two ways. The first one is given in a similar fashion to Chas-Sullivan's string topology. The second one is defined on the Hochschild homology associated with a cyclic, multiplicative operad of graded modules. The latter can be applied to Bousfield-Salvatore spectral sequence converging to the homology of the space of framed long knots. Conjecturally these two structures coincide with each other.

==> nbd.tex <==
%WinTpicVersion4.10
\unitlength 0.1in
\begin{picture}( 18.7000,  8.6500)(  7.3000,-16.0000)
% CIRCLE 2 2 3 0 Black White
% 4 2000 1200 2400 1200 2400 1200 2400 1200
% 
{\color[named]{Black}{%
\special{pn 8}%
\special{ar 2000 1200 400 400  0.0000000 0.0300000}%
\special{ar 2000 1200 400 400  0.1200000 0.1500000}%
\special{ar 2000 1200 400 400  0.2400000 0.2700000}%
\special{ar 2000 1200 400 400  0.3600000 0.3900000}%
\special{ar 2000 1200 400 400  0.4800000 0.5100000}%
\special{ar 2000 1200 400 400  0.6000000 0.6300000}%
\special{ar 2000 1200 400 400  0.7200000 0.7500000}%
\special{ar 2000 1200 400 400  0.8400000 0.8700000}%
\special{ar 2000 1200 400 400  0.9600000 0.9900000}%
\special{ar 2000 1200 400 400  1.0800000 1.1100000}%
\special{ar 2000 1200 400 400  1.2000000 1.2300000}%
\special{ar 2000 1200 400 400  1.3200000 1.3500000}%
\special{ar 2000 1200 400 400  1.4400000 1.4700000}%
\special{ar 2000 1200 400 400  1.5600000 1.5900000}%
\special{ar 2000 1200 400 400  1.6800000 1.7100000}%
\special{ar 2000 1200 400 400  1.8000000 1.8300000}%
\special{ar 2000 1200 400 400  1.9200000 1.9500000}%
\special{ar 2000 1200 400 400  2.0400000 2.0700000}%
\special{ar 2000 1200 400 400  2.1600000 2.1900000}%
\special{ar 2000 1200 400 400  2.2800000 2.3100000}%
\special{ar 2000 1200 400 400  2.4000000 2.4300000}%
\special{ar 2000 1200 400 400  2.5200000 2.5500000}%
\special{ar 2000 1200 400 400  2.6400000 2.6700000}%
\special{ar 2000 1200 400 400  2.7600000 2.7900000}%
\special{ar 2000 1200 400 400  2.8800000 2.9100000}%
\special{ar 2000 1200 400 400  3.0000000 3.0300000}%
\special{ar 2000 1200 400 400  3.1200000 3.1500000}%
\special{ar 2000 1200 400 400  3.2400000 3.2700000}%
\special{ar 2000 1200 400 400  3.3600000 3.3900000}%
\special{ar 2000 1200 400 400  3.4800000 3.5100000}%
\special{ar 2000 1200 400 400  3.6000000 3.6300000}%
\special{ar 2000 1200 400 400  3.7200000 3.7500000}%
\special{ar 2000 1200 400 400  3.8400000 3.8700000}%
\special{ar 2000 1200 400 400  3.9600000 3.9900000}%
\special{ar 2000 1200 400 400  4.0800000 4.1100000}%
\special{ar 2000 1200 400 400  4.2000000 4.2300000}%
\special{ar 2000 1200 400 400  4.3200000 4.3500000}%
\special{ar 2000 1200 400 400  4.4400000 4.4700000}%
\special{ar 2000 1200 400 400  4.5600000 4.5900000}%
\special{ar 2000 1200 400 400  4.6800000 4.7100000}%
\special{ar 2000 1200 400 400  4.8000000 4.8300000}%
\special{ar 2000 1200 400 400  4.9200000 4.9500000}%
\special{ar 2000 1200 400 400  5.0400000 5.0700000}%
\special{ar 2000 1200 400 400  5.1600000 5.1900000}%
\special{ar 2000 1200 400 400  5.2800000 5.3100000}%
\special{ar 2000 1200 400 400  5.4000000 5.4300000}%
\special{ar 2000 1200 400 400  5.5200000 5.5500000}%
\special{ar 2000 1200 400 400  5.6400000 5.6700000}%
\special{ar 2000 1200 400 400  5.7600000 5.7900000}%
\special{ar 2000 1200 400 400  5.8800000 5.9100000}%
\special{ar 2000 1200 400 400  6.0000000 6.0300000}%
\special{ar 2000 1200 400 400  6.1200000 6.1500000}%
\special{ar 2000 1200 400 400  6.2400000 6.2700000}%
}}%
% STR 2 0 3 0 Black White
% 4 1700 1030 1700 1130 5 0 0 0
% $\iota$
\put(17.0000,-11.3000){\makebox(0,0){$\iota$}}%
% VECTOR 2 0 3 0 Black White
% 2 2400 1200 1600 1200
% 
{\color[named]{Black}{%
\special{pn 8}%
\special{pa 2400 1200}%
\special{pa 1600 1200}%
\special{fp}%
\special{sh 1}%
\special{pa 1600 1200}%
\special{pa 1668 1220}%
\special{pa 1654 1200}%
\special{pa 1668 1180}%
\special{pa 1600 1200}%
\special{fp}%
}}%
% STR 2 0 3 0 Black White
% 4 2400 700 2400 800 5 0 0 0
% $g(z)$
\put(24.0000,-8.0000){\makebox(0,0){$g(z)$}}%
% STR 2 0 3 0 Black White
% 4 1550 800 1550 900 5 0 0 0
% $B_{\epsilon}$
\put(15.5000,-9.0000){\makebox(0,0){$B_{\epsilon}$}}%
% STR 2 0 3 0 Black White
% 4 2600 900 2600 1000 2 0 0 0
% $g(z)(t)$
\put(26.0000,-10.0000){\makebox(0,0)[lb]{$g(z)(t)$}}%
% STR 2 0 3 0 Black White
% 4 2400 1200 2400 1300 1 0 0 0
% $p(g(z)(t))=\iota (s_z(t))$
\put(24.0000,-13.0000){\makebox(0,0)[lt]{$p(g(z)(t))=\iota (s_z(t))$}}%
% STR 2 0 3 0 Black White
% 4 2300 1100 2300 1200 5 0 0 0
% $\bullet$
\put(23.0000,-12.0000){\makebox(0,0){$\bullet$}}%
% FUNC 2 0 3 0 Black White
% 10 1600 800 2400 1600 2000 1200 2400 1200 2000 800 1640 800 2360 1600 0 4 0 0 0 0
% x^3
{\color[named]{Black}{%
\special{pn 8}%
\special{pa 1600 1600}%
\special{pa 1606 1586}%
\special{pa 1620 1544}%
\special{ip}%
\special{pa 1640 1492}%
\special{pa 1650 1468}%
\special{pa 1686 1396}%
\special{pa 1696 1378}%
\special{pa 1700 1370}%
\special{pa 1706 1360}%
\special{pa 1710 1352}%
\special{pa 1716 1346}%
\special{pa 1720 1338}%
\special{pa 1736 1316}%
\special{pa 1760 1286}%
\special{pa 1776 1272}%
\special{pa 1786 1262}%
\special{pa 1806 1246}%
\special{pa 1816 1240}%
\special{pa 1820 1236}%
\special{pa 1826 1234}%
\special{pa 1830 1232}%
\special{pa 1836 1228}%
\special{pa 1840 1226}%
\special{pa 1846 1224}%
\special{pa 1866 1216}%
\special{pa 1870 1214}%
\special{pa 1876 1212}%
\special{pa 1886 1210}%
\special{pa 1890 1208}%
\special{pa 1906 1206}%
\special{pa 1910 1206}%
\special{pa 1920 1204}%
\special{pa 1926 1204}%
\special{pa 1930 1202}%
\special{pa 1956 1202}%
\special{pa 1960 1200}%
\special{pa 2060 1200}%
\special{pa 2066 1198}%
\special{pa 2080 1198}%
\special{pa 2090 1196}%
\special{pa 2096 1196}%
\special{pa 2110 1192}%
\special{pa 2116 1190}%
\special{pa 2126 1188}%
\special{pa 2130 1186}%
\special{pa 2136 1186}%
\special{pa 2156 1178}%
\special{pa 2160 1174}%
\special{pa 2166 1172}%
\special{pa 2170 1170}%
\special{pa 2176 1168}%
\special{pa 2180 1164}%
\special{pa 2186 1160}%
\special{pa 2196 1154}%
\special{pa 2216 1138}%
\special{pa 2220 1134}%
\special{pa 2226 1130}%
\special{pa 2240 1114}%
\special{pa 2266 1084}%
\special{pa 2280 1064}%
\special{pa 2286 1056}%
\special{pa 2290 1048}%
\special{pa 2296 1040}%
\special{pa 2300 1032}%
\special{pa 2306 1024}%
\special{pa 2316 1006}%
\special{pa 2336 966}%
\special{pa 2350 932}%
\special{pa 2360 908}%
\special{fp}%
\special{pa 2380 858}%
\special{pa 2396 816}%
\special{pa 2400 800}%
\special{ip}%
}}%
% STR 2 0 3 0 Black White
% 4 2300 930 2300 1030 5 0 0 0
% $\bullet$
\put(23.0000,-10.3000){\makebox(0,0){$\bullet$}}%
% VECTOR 3 0 3 0 Black White
% 2 2300 1030 2300 1190
% 
{\color[named]{Black}{%
\special{pn 4}%
\special{pa 2300 1030}%
\special{pa 2300 1190}%
\special{fp}%
\special{sh 1}%
\special{pa 2300 1190}%
\special{pa 2320 1124}%
\special{pa 2300 1138}%
\special{pa 2280 1124}%
\special{pa 2300 1190}%
\special{fp}%
}}%
% LINE 3 0 3 0 Black White
% 2 2330 1030 2600 1000
% 
{\color[named]{Black}{%
\special{pn 4}%
\special{pa 2330 1030}%
\special{pa 2600 1000}%
\special{fp}%
}}%
% STR 2 0 3 0 Black White
% 4 2000 1100 2000 1200 5 0 0 0
% $\bullet$
\put(20.0000,-12.0000){\makebox(0,0){$\bullet$}}%
% STR 2 0 3 0 Black White
% 4 2000 1000 2000 1100 5 0 0 0
% $\infty$
\put(20.0000,-11.0000){\makebox(0,0){$\infty$}}%
% FUNC 1 0 3 0 Black White
% 9 1600 800 2000 1600 2000 1200 2400 1200 2000 800 1600 800 2000 1600 0 4 0 0
% ((x^3)*exp(1/(0.4+x)))/(exp(1/(0.4+x))+exp(1/(-x-0.9)))
{\color[named]{Black}{%
\special{pn 13}%
\special{pa 1600 1200}%
\special{pa 1636 1200}%
\special{fp}%
\special{pa 1646 1480}%
\special{pa 1650 1468}%
\special{pa 1666 1436}%
\special{pa 1700 1366}%
\special{pa 1706 1354}%
\special{pa 1710 1342}%
\special{pa 1716 1330}%
\special{pa 1726 1302}%
\special{pa 1730 1286}%
\special{pa 1740 1256}%
\special{pa 1746 1242}%
\special{pa 1750 1230}%
\special{pa 1756 1222}%
\special{pa 1760 1214}%
\special{pa 1766 1210}%
\special{pa 1770 1206}%
\special{pa 1780 1202}%
\special{pa 1786 1202}%
\special{pa 1790 1200}%
\special{pa 1836 1200}%
\special{fp}%
\special{pa 1846 1224}%
\special{pa 1866 1216}%
\special{pa 1870 1214}%
\special{pa 1876 1212}%
\special{pa 1886 1210}%
\special{pa 1890 1208}%
\special{pa 1906 1206}%
\special{pa 1910 1206}%
\special{pa 1920 1204}%
\special{pa 1926 1204}%
\special{pa 1930 1202}%
\special{pa 1956 1202}%
\special{pa 1960 1200}%
\special{pa 2000 1200}%
\special{fp}%
}}%
% STR 2 0 3 0 Black White
% 4 1400 1300 1400 1400 4 0 0 0
% $\tilde{g}(z)$
\put(14.0000,-14.0000){\makebox(0,0)[rt]{$\tilde{g}(z)$}}%
% LINE 3 0 3 0 Black White
% 2 1400 1400 1740 1240
% 
{\color[named]{Black}{%
\special{pn 4}%
\special{pa 1400 1400}%
\special{pa 1740 1240}%
\special{fp}%
}}%
% STR 2 0 3 0 Black White
% 4 1800 1250 1800 1350 1 0 0 0
% $g(z)$
\put(18.0000,-13.5000){\makebox(0,0)[lt]{$g(z)$}}%
% LINE 3 0 3 0 Black White
% 2 1800 1400 1800 1250
% 
{\color[named]{Black}{%
\special{pn 4}%
\special{pa 1800 1400}%
\special{pa 1800 1250}%
\special{fp}%
}}%
% LINE 3 0 3 0 Black White
% 2 2420 1320 2300 1200
% 
{\color[named]{Black}{%
\special{pn 4}%
\special{pa 2420 1320}%
\special{pa 2300 1200}%
\special{fp}%
}}%
\end{picture}%

